Context-Aware Zero-Shot Learning for Object Recognition

Zero-Shot Learning (ZSL) aims at classifying unlabeled objects by leveraging auxiliary knowledge, such as semantic representations. A limitation of previous approaches is that only intrinsic properties of objects, e.g. their visual appearance, are taken into account while their context, e.g. the surrounding objects in the image, is ignored. Following the intuitive principle that objects tend to be found in certain contexts but not others, we propose a new and challenging approach, context-aware ZSL, that leverages semantic representations in a new way to model the conditional likelihood of an object to appear in a given context. Finally, through extensive experiments conducted on Visual Genome, we show that contextual information can substantially improve the standard ZSL approach and is robust to unbalanced classes.

==> models.tex <==

\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;} 

\begin{table}[h]
    \centering
    \vspace{-0.3cm}
        \caption{Context models}
    \begin{tabularx}{\columnwidth}{l | c c c}
        \multicolumn{1}{c|}{Context} & Word emb. & CNN rep. & CNN rep.  \\
        \multicolumn{1}{c|}{Model} & known obj. & known obj. & unknown obj.  \\
        \hline
        %$\varnothing$ & & &\\
        $ K_t$ & \checkmark& &\\
        $K_v$ & & \checkmark  \\
        $ U_v$ & & &\checkmark\\
        $ K_{v \phantom{+t}} + U_v$& &\checkmark  &\checkmark\\
        $ K_{t \phantom {+v}} + U_v$ & \checkmark& &\checkmark\\
        $K_{v+t}+U_v$ & \checkmark& \checkmark& \checkmark\\
    \end{tabularx}
    \label{models}
\end{table}


==> scenarios.tex <==
\newlength{\lfont}
\setlength{\lfont}{9.5pt}
\begin{table}[h]
    \centering
        \caption{MFR performances of our approach for different context models and components configurations. $p_{sup}=50\%$. As a comparison, please note that $\mathcal{V} + \mathcal{P}$ has MFR$=10.72\%$ (resp. $2.64\%$) for unkown (resp. known) objects.}
        \begin{tabularx}{\columnwidth}{l | c c | c c}
        
        & \multicolumn{2}{c|}{Unknown objects} & \multicolumn{2}{c}{Known objects}\\
        
      Context & {\fontsize{\lfont}{0}\selectfont $\mathcal{C} + \mathcal{P}$} & {\fontsize{\lfont}{0}\selectfont $\mathcal{C} + \mathcal{V} + \mathcal{P}$} & {\fontsize{\lfont}{0}\selectfont $\mathcal{C} + \mathcal{P}$} & {\fontsize{\lfont}{0}\selectfont $\mathcal{C} + \mathcal{V} + \mathcal{P}$} \\
        \hline
     $K_t$  & 14.35 & 8.96 & 4.25 & 1.92 \\ 
      $K_v$ & 13.00 & 9.01 & 3.81 & 2.05 \\
      $U_v$& 12.59 & 9.00 & 4.24 & 2.13 \\
      $K_{t \phantom{+t}} +U_v$   &  \\ 
     $K_{v\phantom{+t}}+U_v$   & 11.88 & 8.60 & 3.49 & 1.93 \\ 
       $K_{v+t}+U_v$ &  \textbf{11.24} & \textbf{8.31} & \textbf{3.17} & \textbf{1.79}  \\ 
    \end{tabularx}

    \label{full_table_scenarios}
\end{table}


==> table_50.tex <==

\begin{table*}[h]
    \centering
        \caption{Comparison of the baselines and scenarios, with $p_{sup}=50\%$, i.e.  ${|\mathcal{K}| = |\mathcal{U}| = 50\%  |\mathcal{O}|}$. MFR results are given in percentage. Oracle results are written in italics; they are not taken into account to determine the best scores, written in bold. }
        \begin{tabularx}{\textwidth}{l l c | Y Y Y Y | Y Y Y Y}
       & & & \multicolumn{4}{c|}{Unknown objects} & \multicolumn{4}{c}{Known objects}\\
        %\cline{3-6}
        %\hline
      %  & & - & $\mathcal{P}$ & $\mathcal{V}$ & $\mathcal{V} + \mathcal{P}$ & - & $\mathcal{P}$ & $\mathcal{V}$ & $\mathcal{V} + \mathcal{P}$ \\
       % \cline{3-10}
       % True prior & Oracle & - & 10.50 & - & - & - & 10.67 & - & - \\
      %  Learned prior & & - & 10.60 & - & - & -  & 23.71 & - & - \\
      %  \hline
      &  & \multirow{2}{*}{Context} & \multirow{2}{*}{$\mathcal{C}$} & \multirow{2}{*}{$\mathcal{C} + \mathcal{P}$} & \multirow{2}{*}{$\mathcal{C}+\mathcal{V}$} & $\mathcal{C} + \mathcal{V} + \mathcal{P}$ & \multirow{2}{*}{$\mathcal{C}$} & \multirow{2}{*}{$\mathcal{C} + \mathcal{P}$} & \multirow{2}{*}{$\mathcal{C} + \mathcal{V}$} & $\mathcal{C} + \mathcal{V} + \mathcal{P}$  \\
        \hline
    \multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{Baselines}}}  &  Random & - &100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 \\
       & True prior (Oracle) & Bayes & \textit{10.70} & \textit{5.35} & \textit{6.03} & \textit{3.40} & \textit{10.44} & \textit{4.83} & \textit{4.01} & \textit{2.11} \\
     &  Textual & Bayes &  \\
     &  DeViSE & $\varnothing$  & - & 23.71 & 25.79 & 10.72 & - & 10.60 & 10.90 & 2.64\\
     &  True Prior (Oracle) & $\varnothing$  & - & \textit{10.67} & \textit{25.79} & \textit{4.92}& - & \textit{10.50} & \textit{10.90} & \textit{2.63} \\
     &  Image  &$I$  & 38.73 & 13.06 & 22.87 & 9.19& 18.75 & 4.18 & 8.13 & 2.13 \\ %"/net/edwards/zablocki/zsl/2018-12-22_14-07-35.185882/"
        %Bayes model + True prior (full) & Oracle & 6.70 & 4.00 & - & - & 7.52 & 4.78 & - & - \\
      &  Word all  (Oracle) & $K_w+U_w$ & \textit{26.88} & \textit{11.15} & \textit{17.32} & \textit{7.57}& \textit{19.52} & \textit{4.10} & \textit{7.60} & \textit{2.53}  \\ % not finished but almost  /net/chic/zablocki/zsl/2018-12-28_11-07-33.650881/
        \hline
    \multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{Our models}}}  &  Word . known  & $K_w$ & 39.88 & 14.35 & 20.98 & 8.96  & 24.14 & 4.25 & 6.92 & 1.92\\ % /net/chic/zablocki/zsl/2018-12-18_15-00-33.276174/
     &   CNN known  & $K$ & \\
     &   CNN unknown  & $U$& \\
        %CNN all  (fixed) &$K+U$ & 22.94 & 4.15 & 8.86 & 2.18 & 36.53 & 13.24 & 21.95 & 9.19 \\ % "/net/edwards/zablocki/zsl/2018-12-25_12-41-20.151637/" 
        %CNN all  (with devise) &$K+U$ & 22.11 & 4.11 & 8.95 & 2.67 & 35.14 & 12.44 & 22.00 & 9.07 \\ %/net/edwards/zablocki/zsl/2018-12-24_10-25-43.228452/
      &  CNN all &$K+U$  & 35.85 & 11.88 & 21.85 & 8.60& 18.01 & 3.49 & 7.98 & 1.93 \\ % warning not best checkpoint "/net/edwards/zablocki/zsl/2018-12-28_11-04-04.664096/train/my-model-3246671"
        %CNN unseen + W2V seen & & \\ 
        %CNN full + W2V seen & & 21.13 & 3.84 & 7.06 & 1.92 & 36.78 & 13.50 & 21.48 & 9.08 \\ % /net/pas/zablocki/zsl/2018-12-24_10-41-12.402653
        %CNN full (with devise) + W2V seen & & 19.40 & 3.57 & 7.08 & 1.92 & 34.07 & 12.23 & 21.26 & 8.81 \\ % "/net/titan/zablocki/zsl/2018-12-24_10-41-42.249027/" can maybe wait more
       & CNN all + Word  known  & $K+K_w+U$ & \textbf{32.71} & \textbf{11.24} & \textbf{20.30} & \textbf{8.31}& \textbf{16.49} & \textbf{3.17} & \textbf{6.51} & \textbf{1.79}  \\ % 1. 1. for aggregate + w2v_seen % 1.0, 0.04, 0.09 for devise + aggregate + w2v_seen % 1.0 0.5 0.4 for prior + aggregate + w2v_seen % 1.0 4.375 0.35 0.3125 for prior + devise + aggregate  + w2v_seen 
        %\hline 
        %Bayes + Learned prior (seen) &  & 10.44 & 4.88 & 4.01 & 2.13 & 10.70 & 7.24 & 6.03 & 4.43 \\
    \end{tabularx}

    \label{full_table}
\end{table*}

% Eval baseline image --> TODO remake splits train valid test that work...
% W2V FULL --> Eval the last one 

% WAIT FOR CNN OTHER CONTEXT
% CNN seen
% W2V seen & CNN unseen

% TODO
% True prior cheating -> eval
% Random context -> relaunch
% Co-occurrence naive-bayes Oracleing

% TODO
% Relaunch prior 10%
% Prior for 90% -> launched
% Devise for 90%

==> table_50_old.tex <==
\begin{table*}[h]
    \centering
    \begin{tabular}{l l | c c | c c}
        & & \multicolumn{2}{c|}{Seen objects} & \multicolumn{2}{c}{Unseen objects}\\
        %\cline{3-6}
        %\hline
        & & $\mathcal{L_C}$ & $\mathcal{L_C}+\mathcal{L_V}$ & $\mathcal{L_C}$ & $\mathcal{L_C} + \mathcal{L_V}$ \\
        %\cline{3-6}
        \hline
        No context (DeVISE only) & $\mathcal{L_C}=\varnothing$ & - & 4.35 & - & 10.86\\
        \hline
        True Prior (cheating) & & 10.73 & 3.84 & 11.03 & 6.16 \\
        Learned Prior & $\mathcal{L_C}^\text{prior}$ & 10.78 & 3.87 & 24.00 & 10.78 \\
        Random context & $\mathcal{L_C}^\text{random}$ & 10.72 & 3.95 & 25.15 & 10.86 \\
        \hline
        Word2Vec for seen objects & $\mathcal{L_C}^{Sw}$ & 3.42 & 2.30 & 15.21 & 9.04 \\ % TODO modify that
        Word2Vec for unseen objects (cheating) & $\mathcal{L_C}^{Uw}$ & 4.89 & 2.96 & 13.77 & 9.00 \\ % TODO modify that
        Word2Vec for all objects (cheating) & $\mathcal{L_C}^{(S + U)w}$ & 3.24 & 2.32 & 12.40 & 8.53 \\
        \hline
        CNN for seen objects & $\mathcal{L_C}^{S}$ & 4.19 & 2.94 & 14.19 & 9.51\\ % TODO modify that
        CNN for unseen objects & $\mathcal{L_C}^{U}$ & 4.48 & 3.02 & 13.30 & 9.14\\ % TODO modify that
        CNN for all objects & $\mathcal{L_C}^{S + U}$ & 4.03 & 2.92 & 12.82 & 9.05 \\
        \hline
        CNN for unseen objects, Word2Vec for seen objects & $\mathcal{L_C}^{U} + \mathcal{L_C}^{Sw}$ & 3.22 & 2.32 & 13.05 & 8.92 \\ % TODO modify that
        CNN for all objects, Word2Vec for seen objects & $\mathcal{L_C}^{S+U} + \mathcal{L_C}^{Sw}$ & 3.19 & 2.36 & 12.59 & 8.74 \\ % TODO modify that
        \hline
        CNN for all objects, different weights than DeVISE & & 3.65 & 2.68 & 12.84 & 8.81 \\
        %Attention context, Word2Vec for seen objects & $\mathcal{L_C}^{Sw}$ & 1.56 & 1.18 & 4.81 & 4.11 \\ % cheating model
        %Attention context, CNN for all objects & $\mathcal{L_C}^{S + U}$ & 3.11 & 2.74 & 11.15 & 8.95 \\ % cheating model
    \end{tabular}
    \caption{OLD TABLE}
    \label{full_table_old}
\end{table*}

==> table_data.tex <==
%\begin{table}[h]
%    \centering
%        \caption{Number of unique contexts}
%        \begin{tabularx}{\columnwidth}{l| c c c c c}
%        \# unique contexts & [0-8[ & [8, 64[ & [64, 512[ & [512, 4096[ & [4096, 4842[\\
%        \hline
%        \# entities & 4 & 135 & 3175 & 1520 & 8
%        %& & \multicolumn{4}{c|}{Known objects} & \multicolumn{4}{c}{Unknown objects}\\
%    \end{tabularx}
%    \label{table_data}
%\end{table}



==> table_devise_50.tex <==
\begin{table*}[h]
    \centering
    \begin{tabular}{l l | c c c | c c c}
        & & \multicolumn{3}{c|}{Seen objects} & \multicolumn{3}{c}{Unseen objects}\\
        %\cline{3-6}
        %\hline
        & & $\mathcal{P}$ & $\mathcal{V}$ & $\mathcal{V}+\mathcal{P}$ & $\mathcal{P}$ & $\mathcal{V}$ & $\mathcal{V} + \mathcal{P}$ \\
        %\cline{3-6}
        \hline
        Learned prior & & 10.59 & - & - & 23.71 & - & - \\
        \hline
        Devise & & - & 12.45 & 2.90 & - & 26.67 & 10.81 \\
    \end{tabular}
    \caption{MFR results in percentage, obtained when ${|\mathcal{S}| = |\mathcal{U}| = \frac{|\mathcal{O}|}{2}}$}
    \label{devise_table}
\end{table*}

==> table_nb.tex <==
\begin{table}[t]
    \centering
        \caption{MFR performances (given in $\%$) for $p_\text{sup}=50\%$.}
       %\vspace{-0.10cm}
        \begin{tabularx}{\columnwidth}{@{\hspace{0.1pt}} C{0.1pt} @{\hspace{10pt}} O{7.5pt} Q{88pt} @{\hspace{4pt}} | Y Y}
    & & {Model} & Target $\mathcal{T}$ & Source $\mahtcal{S}$ \\
    %& \multicolumn{2}{c|}{Context Model} & Target & Source \\
        \hline
     %&  Oracle: Textual cooc. & Bayes & \textit{27.24} & \textit{23.89} \\ % textual prior
    
     %&  Oracle: Textual cooc. & Bayes & 8.65 & 17.20 \\
    %&  Random & &  100.0 & 100.0 \\
        %\cdashline{2-5}
        \hline
    & DeViSE & $P(.|\mathcal{V})$ & 10.73 & 3.62\\
    & & $P(.|\mathcal{C}_{S_H}, \mathcal{V})$ &  10.11&  3.11 \\ 
    & & $P(\mathcal{C}_{S_H}, \mathcal{V}|.)P(.)$  & 10.07 &  1.85 \\ 
    \end{tabularx}
    \label{full_table}
    \vspace{-0.5cm}
\end{table}

